ALIGN: Word Association Learning for Cultural Alignment in Large Language Models

Large language models (LLMs) exhibit cultural bias from overrepresented viewpoints in training data, yet cultural alignment remains a challenge due to limited cultural knowledge and a lack of exploration into effective learning approaches. We introduce a cost-efficient and cognitively grounded method: fine-tuning LLMs on native speakers' word-association norms, leveraging cognitive psychology findings that such associations capture cultural knowledge. Using word association datasets from native speakers in the US (English) and China (Mandarin), we train Llama-3.1-8B and Qwen-2.5-7B via supervised fine-tuning and preference optimization. We evaluate models' cultural alignment through a two-tier evaluation framework that spans lexical associations and cultural value alignment using the World Values Survey. Results show significant improvements in lexical alignment (16-20% English, 43-165% Mandarin on Precision@5) and high-level cultural value shifts. On a subset of 50 questions where US and Chinese respondents diverge most, fine-tuned Qwen nearly doubles its response alignment with Chinese values (13 to 25). Remarkably, our trained 7-8B models match or exceed vanilla 70B baselines, demonstrating that a few million of culture-grounded associations achieve value alignment without expensive retraining. Our work highlights both the promise and the need for future research grounded in human cognition in improving cultural alignment in AI models.

==> latex/tables/evaluation_datasets.tex <==


\begin{table*}[!t]
    \centering
    \begin{tabular}{l|ccc|p{4cm}|p{4cm}}
        \toprule
        Dataset & Type & Size &Size-Zh &  Construction &Languages\\
        \midrule 
        WVS & Value &  290 & 240? & Mannual\\ 
        CASA & Norm & 618 + 607& 17 + 23 &  LLM + Human Verification& \\ 
        CulturalBench & Norm? & 1227 & 59 & native speaker Written&(45 langauges) US, Zh, Spain, ...\\ 
        MAPS & Proverbs &  & 335 & GPT3.5 generated + native speaker verified & En, Zh, De, Ru, Bn, Id \\ 
        CulturalTrap & &&& \\ 
        \bottomrule
    \end{tabular}
    \caption{The datasets for evaluating various datasets}
    \label{tab:evaluation_datasets}
\end{table*}




==> latex/tables/sukai_original_sft_ppo_results.tex <==


\begin{table*}[ht]
    \footnotesize
    \centering
    \begin{tabular}{cccccccccc}
    \toprule
    \textbf{Label} & \textbf{Model Type} & \textbf{Model Class} & \textbf{SWOW Type} & \textbf{Prec@5} & \textbf{Prec@10} & \textbf{Prec@20} & \textbf{Prec@30} & \textbf{Prec@40} & \textbf{Spearman} \\
    \midrule
    1 & vanilla & qwen & English & 0.6339 & 0.5020 & 0.3668 & 0.2903 & 0.2386 & 0.3726 \\
    2 & SFT & qwen & English & \textbf{0.7617}  & \textbf{0.6517}  & \textbf{0.4958} & \textbf{0.3924}  & \textbf{0.3279}  & \textbf{0.4944}  \\
    3 & PPO only & qwen & English &  0.6371  &  0.5056 &  0.3703  &  0.2918 &  0.2383 & 0.3649  \\
    % 4* & SFT + PPO & qwen & English & 0.7357  & 0.6529  & 0.5364  & 0.4516  & 0.3883  & 0.4624  \\
    4 & vanilla & qwen & Mandarin & 0.4812  & 0.3640  & 0.2547 & 0.1974  & 0.1590  & 0.2893  \\
    5* & SFT & qwen & Mandarin & 0.6889  & 0.5593 & 0.4032  & 0.3253 & 0.2797  & 0.3657  \\
    6 & PPO only & qwen & Mandarin &  0.4967 &  0.3780 &  0.2614 & 0.1983  &  0.1588  &  0.2853 \\
    % 8 & SFT + PPO & qwen & Mandarin & 0.5945  & 0.4837  & 0.3644  & 0.3001 & 0.2603  & 0.3251  \\
    \bottomrule
    \end{tabular}
    \caption{Word Association Generation for Qwen}
    \label{tab:qwen_word_assoc}
\end{table*}

\begin{table*}[ht]
    \footnotesize
    \centering
    \begin{tabular}{cccccccccc}
    \toprule
    \textbf{Label} & \textbf{Model Type} & \textbf{Model Class} & \textbf{SWOW Type} & \textbf{Prec@5} & \textbf{Prec@10} & \textbf{Prec@20} & \textbf{Prec@30} & \textbf{Prec@40} & \textbf{Spearman} \\
    \midrule
    1 & vanilla & llama & English & 0.7548 & 0.6094  & 0.4465  & 0.3554  & 0.2953  & 0.4484  \\
    2* & SFT & llama & English & 0.8754  & 0.7736  & 0.6247  & 0.5143  & 0.4370  & 0.5036  \\
    3 & PPO only & llama & English &  0.7850 &  0.6408 & 0.4686 &  0.3682 & 0.3039 & 0.4677 \\
    % 4 & SFT + PPO & llama & English & 0.8161  & 0.7030  & 0.5566  & 0.4605  & 0.3952  & 0.4815  \\
    4 & vanilla & llama & Mandarin & 0.2602  & 0.1818  & 0.1088  & 0.0759  & 0.0577  & 0.2235  \\
    5* & SFT & llama & Mandarin & 0.6897  & 0.5565  & 0.4003  & 0.3200  & 0.2777  & 0.3355  \\
    6 & PPO only & llama & Mandarin &  0.2716 &  0.1951 &  0.1189 &  0.0842 &  0.0638 & 0.2371 \\
    % 8 & SFT + PPO & llama & Mandarin & 0.5389  & 0.4308  & 0.3175  & 0.2554  & 0.2205  & 0.3147  \\
    \bottomrule
    \end{tabular}
    \caption{Word Association Generation for Llama}
    \label{tab:llama_word_assoc}
\end{table*}

\subsection*{Ranking Task Evaluation}
\begin{table*}[ht]
    \centering
    \begin{tabular}{ccccc}
    \toprule
    \textbf{Label} & \textbf{SWOW Type} & \textbf{Model Class} & \textbf{Model Type} & \textbf{Spearman's Score} \\
    \midrule
    1 & English & qwen & vanilla & 0.2924 \\
    2 & English & qwen & SFT & 0.5776 \\
    3 & English & qwen & PPO only & 0.3218 \\
    % 4* & English & qwen & SFT + PPO & 0.6269 \\
    4 & Mandarin & qwen & vanilla & 0.2919 \\
    5 & Mandarin & qwen & SFT & -0.5518 \\
    6* & Mandarin & qwen & PPO only & 0.3237 \\
    % 8 & Mandarin & qwen & SFT + PPO & -0.3362 \\
    \bottomrule
    \end{tabular}
    \caption{Qwen Model Performance on Ranking Task}
    \label{tab:qwen_performance}
\end{table*}

\begin{table*}[ht]
    \centering
    \begin{tabular}{ccccc}
    \toprule
    \textbf{Label} & \textbf{SWOW Type} & \textbf{Model Class} & \textbf{Model Type} & \textbf{Spearman's Score} \\
    \midrule
    1 & English & llama & vanilla & 0.2415 \\
    2 & English & llama & SFT & -0.2832 \\
    3* & English & llama & PPO only & 0.2708 \\
    % 4 & English & llama & SFT + PPO & -0.3226 \\
    4 & Mandarin & llama & vanilla & 0.2116 \\
    5 & Mandarin & llama & SFT & -0.9960 \\
    6* & Mandarin & llama & PPO only & 0.2260 \\
    % 8 & Mandarin & llama & SFT + PPO & -0.9979 \\
    \bottomrule
    \end{tabular}
    \caption{Llama Model Performance on Ranking Task}
    \label{tab:llama_performance}
\end{table*}


==> latex/tables/sukai_original_training.tex <==
\section{Fine-tuning LLMs on cultural associations}
\textcolor{red}{@sukai}

% \begin{color}{orange}
% \begin{itemize}
%     \item Goal, hypothesis, task design
%     \item how did we train them? on what data (data statistics)?
%     \item how did we evaluate them? why? how does the performance look like? what does the results mean? 
%     \item anything you think is important ...
% \end{itemize}    
% \end{color}
\subsection{Datasets}
We use the small world of words datasets to train our models.  Specifically, we use the English SWOW (\swen)\cite{de2019small} and Mandarin SWOW (\swzh) \cite{li2024large}.
\swen was collected during \textcolor{red}{2011-2019}. 
\swzh was collected during \textcolor{red}{201x-2023?}.
Both of them include 12K cues that are used as stimuli. 
\swen contains xx responses, while \swzh contains xx responses (due to fewer participants being involved).
We randomly split 80\% of the data for training and remaining 10\% for validation and 10\% hold-out to test the model performance.  




\definecolor{sukaicolor}{RGB}{163,193,244}

% Create a style for highlighting paragraphs
\mdfdefinestyle{sukaihighlight}{%
    backgroundcolor=sukaicolor,
    linewidth=0pt,
    innerleftmargin=5pt,
    innerrightmargin=5pt,
    innertopmargin=5pt,
    innerbottommargin=5pt
}

\begin{mdframed}[style=sukaihighlight]
    Comment: I will use fine-tuning to replace the term training, and also RLHF is considered as framework for fine-tuning too, see \citet{xiao2025on} introduction.
\end{mdframed}

Like with RAG, we assume that word associations effectively reflect cultural values. However, instead of relying on RAG, in this section, we discuss directly fine-tuning the LLMs on the word association data.

Fine-tuning LLMs directly on word association datasets offers distinct advantages over using RAG to align models with cultural values. While RAG can be seen as providing additional context to guide a model's decisions at inference time, fine-tuning reshapes the model's behavior by adjusting its weight parameters. This approach has two key benefits:

\textbf{Independence from external KB:} \quad Fine-tuning eliminates the need for an external retrieval system during inference. RAG relies on real-time access to a knowledge base, which may not always be \emph{available} and can significantly slow down inference due to retrieval latency. In contrast, a fine-tuned model carries its learned associations internally, making it faster and more self-contained.

\textbf{Generalization beyond the dataset:}\quad Fine-tuning enables the model to generalize to unseen examples by learning patterns and semantic relationships during training. For example, since ``gorilla'' and ``monkey'' are close in the word embedding space due to their shared features, a model fine-tuned on ``monkey'' or other nearby words—whether as cue words or associations—can implicitly infer associations for ``gorilla,'' even if it's absent from the dataset. (As a side note, a vector database in a retrieval-based approach could also leverage embedding similarities to achieve this, but that's beyond the scope of this work.) In contrast, RAG's performance is heavily dependent on the quality and coverage of the retrieval dataset. If the retrieved context is poor or incomplete, the model's performance suffers. 

In the following sections, we discuss the types of fine-tuning techniques and the associated task designs we employ for LLMs to learn word associations.

\subsection{Supervised Fine-tuning}

To provide context, we consider autoregressive LMs such as the GPT \citep{DBLP:conf/nips/BrownMRSKDNSSAA20} and LLaMA \citep{grattafiori2024llama3herdmodels} series, which generate tokens in a left-to-right, autoregressive manner. Let $\mathbf{x}{< i}$ be the first $i - 1$ tokens of a sequence $\mathbf{x}$, and let $x_i$ be the $i$-th token. The probability that the LLM predicts token $x_i$ at position $i$ can be written as $LM\theta(\hat x_i = x_i \mid \mathbf{x}{< i})$, where $LM\theta(\cdot)$ is the model's probability distribution over the vocabulary, and $\theta$ represents the model parameters.

We implement \emph{the word association prediction task} directly in the supervised fine-tuning (SFT) framework. Given a training example $x = \langle c, \mathbf{w} \rangle$, where $c$ is a cue word and $\mathbf{w} = \langle w_1, w_2, \ldots, w_n \rangle$ is a list of associated words, the model is trained to generate the associated words $\mathbf{w}$ conditioned on the cue word $c$. The objective of SFT is to maximize the likelihood of the training data, which is formalized as:

\begin{equation} 
    J(\theta) = \max_{\theta} \mathbb{E}_{\mathbf{x} \sim \mathcal{X}} \left[ \sum_{i=1}^{|\mathbf{x}|} \log LM_\theta(x_i \mid \mathbf{x}_{< i}) \right] 
\end{equation}

where $\mathcal{X}$ denotes the training dataset, and $|\mathbf{x}|$ is the length of the token sequence.

While this formulation captures the core learning objective, in practice we reformat each training instance into a more natural, instruction-style prompt that aligns with how LLMs are typically used. For example, we add constraints to the prompt to further guide the model's generation process, such as ``do not generate words conditioned on the presence of other words, but focus solely on the cue word.'' See \aref{appendix:sft_prompt_instructions} for details.


\subsection{PPO training}

To further align LLMs with culturally-informed word associations, we explore reinforcement learning from human feedback (RLHF), using the Proximal Policy Optimization (PPO) algorithm \citep{schulman2017proximal}. RLHF has proven to be a powerful technique for fine-tuning LLMs by aligning them with preferences defined by a reward model, which is either trained on human feedback or based on predefined rules \citep{DBLP:conf/nips/Ouyang0JAWMZASR22, deepseekai2025deepseekr1incentivizingreasoningcapability}. Recent studies have demonstrated that RLHF outperforms supervised fine-tuning (SFT) in improving LLMs' reasoning abilities. One explanation is that RLHF encourages exploration beyond the explicit solutions present in the training set, whereas SFT primarily trains the model to mimic human-provided data, leading to shallow imitation \citep{havrilla2024teaching, chu2025sft}. Another perspective frames the difference between SFT and RLHF through an imitation learning lens: SFT minimizes \emph{forward KL divergence} between the model and the response distribution, while RLHF minimizes \emph{reverse KL divergence} \citep{xiao2025on} and exhibits \emph{Mode-Seeking Behavior}. This behavior ensures that the model \emph{focuses} on a particular mode of the response distribution rather than attempting to cover the entire distribution. Such behavior makes RLHF particularly suitable for reasoning tasks that demand precise and accurate answers. For further details on the differences between these fine-tuning approaches, we refer readers to \citet{xiao2025on}.

In our case, instead of human preferences, we use an automatic reward function designed to reflect the fulfillment of designed tasks. Before we turn into the task design, we first introduce the three components of RLHF framework: 
\begin{enumerate}
    \item a language model (policy) $LM_\theta$ generating candidate outputs,  
    \item a reward model $r(q, a)$ evaluating those outputs, where $q$ is the question and $a$ is the generated answer, and
    \item a reinforcement learning algorithm (e.g., PPO) that updates the model to maximize the received reward.
\end{enumerate}


Formally, RLHF fine-tunes the language model \( LM_\theta \) by optimizing the following objective:

\begin{flalign}
    &\max_{\theta} \mathbb{E}_{a \sim LM_\theta(a \mid q)} \left[ r(q, a) \right] \nonumber\\
    &- \beta D_{\text{KL}} \left[ LM_\theta(a \mid q)  ||  LM_{\text{ref}}(a \mid q) \right]
\end{flalign}
where $ LM_{\text{ref}}$ is a frozen reference model (typically the initial SFT model), and \( \beta \) is a scaling factor controlling the KL penalty that discourages large divergences from the reference model so as to maintain the model stability. 

We conducted preliminary experiments with multiple task formats to determine the most effective design for PPO training:

\textbf{Free-form word association generation}\quad Initially, we framed the task as the same open-ended generation as SFT, where the model was asked to predict associated words given a cue word. However, this setup proved too unconstrained: the model is allowed to generate unrelated or irrelevant associations, making the reward signal noisy and the gradients unstable.

\textbf{Multiple-choice question (MCQ) format}\quad We then explored a classification-style task where the model selected the most strong option of word associations from a list of candidates. However, this task turned out to be too easy for LLMs, with near-perfect accuracy even before fine-tuning, leaving minimal gradient signal for PPO to improve upon.

\textbf{Ranking-based format}\quad Ultimately, we settled on a ranking task, where the model was asked to rank a list of association words of a cue word based on its frequency in the SWOW dataset. This design offers a middle ground: (1) It is more structured and constrained than free-form generation, improving training stability and (2) It is more challenging than MCQ, providing useful reward gradients for learning.  

The reward function evaluates the alignment between the model's ranked list and ground truth rankings using Spearman's rank correlation coefficient. See \aref{appendix:ppo_reward_details} for details.

While our main results focus on evaluating cultural alignment in downstream tasks, we also assess the LLMs’ performance on the training tasks themselves—namely, supervised fine-tuning (SFT) for word association prediction and PPO training for ranking tasks. These results provide hints into whether models have successfully learned word association patterns during fine-tuning. Due to space constraints, detailed evaluation results are reported in \aref{appendix:sft_ppo_eval}.

\end{CJK*}
